A Survey of Robotics and Emotion: Classifications and Models of Emotional Interaction

As emotion plays a growing role in robotic research it is crucial to develop methods to analyze and compare among the wide range of approaches. To this end we present a survey of 1427 IEEE and ACM publications that include robotics and emotion. This includes broad categorizations of trends in emotion input analysis, robot emotional expression, studies of emotional interaction and models for internal processing. We then focus on 232 papers that present internal processing of emotion, such as using a human's emotion for better interaction or turning environmental stimuli into an emotional drive for robotic path planning. We conducted constant comparison analysis of the 232 papers and arrived at three broad categorization metrics; emotional intelligence, emotional model and implementation, each including two or three subcategories. The subcategories address the algorithm used, emotional mapping, history, the emotional model, emotional categories, the role of emotion, the purpose of emotion and the platform. Our results show a diverse field of study, largely divided by the role of emotion in the system, either for improved interaction, or improved robotic performance. We also present multiple future opportunities for research and describe intrinsic challenges common in all publications.

==> sparetext.tex <==
While I have some minor suggestions for improvements, I
believe the paper should be accepted and is currently even
under-stating its contribution it could make to the HRI
community. 
The categories developed to describe and analyze
the related work as presented in Fig. 2 could very well be
suggested as a starting point of a general classification
of literature related to emotions in robotics, which makes
the paper very relevant for the past and future research
int his area. 

% https://scholar.google.com/citations?view_op=top_venues&hl=en&vq=eng_robotics

\subsection{Robotic Platforms}
I could in the future describe more specific platforms.
Using only ACM and IEEE publications, the paper
lacks the most significant work in the field of emotion
such as EMA, Fatima, WASABI, EEGS, etc.

In section F, under platforms, it seems very weird to me
that Emys-type robot was not used in any publications.
While one main feature of Emys ("Emotive" headY System) is
representing emotions by its facial expressions. 



\subsubsection{Unused Categories}
The previous categories all emerged through constant comparison analysis, with many changes and developments occurring through the process. Two categories that were eventually discarded were perceived and evoked emotion and the project stage. Comparing whether the role of emotion 

Perceived vs evoked emotion, 
project stage.  

interesting, but both too blurry to be conclusive. 


\subsubsection{ LOG-LINEAR ANALYSIS}
DISCUSS LOG-LINEAR ANALYSIS

LOGLINEAR MODEL JUST 2 PARAGRAPHS
https://data.library.virginia.edu/an-introduction-to-loglinear-models/

LOG LINEAR Analysis?


Possible hypothesis:
LOG LINEAR
Internal process uses a smaller amount of emotions

Different methods for performance and interaction?

Log Linear compare Interaction type with Emotions
And Interaction type with Input/Output

Will be a relationship between
model used, 
amount of emotions
purpose
Input and output



Gut feeling ideas from looking through the data:
No relationship between role of emotion, purpose and type of robot
Emotional 
Ideas not backed - no relationship between role, purpose and robot

% https://data.library.virginia.edu/an-introduction-to-loglinear-models/

\subsubsection{More Descriping Signalling}
signalling - may get too deep.
\cite{jung2017affective}


\subsection{Anthropomorphism}
Some very false anthropomorphizing. 
Describe the robot as having emotion, and feeling frustrated Saying the robot is sad when something bad happens and it corrects its path without any emotional model is bad
Or in A Hybrid Robot Navigation Approach Based on Partial Planning and Emotion-Based Behavior Coordination -- describes as happy when it sees a target, when there’s not really any clear emotion	

Real Emotions Don’t Stand Still:
Toward Ecologically Viable Representation of Affective Interaction
could use these points to expand




\subsection{extra figures}
\begin{figure}[h]
  \centering
\includegraphics[width=8cm]{images/emotionmodels.png}
  \caption{Emotional Models Count}
  \label{fig:emotionalmodelscount}
\end{figure}

% Figure \ref{fig:emotionalmodelscount} shows the range of emotional models used across all publications. 


\subsection{Emotions not used}
This list of emotion models is very
limited. A large number of computational models of emotion
have been implemented based on emotion theories such as
Appraisal Theory (OCC, Scherer, Lazarus, Roseman, etc.),
Dimensional Theories (Circumplex, Plutchik, Lovheim, etc.),
Physiological Theories (James, etc.)


\subsection{Expand Description of Process}
-	In the Methodology section, authors state ìWe used
constant comparison analysis to build categories and
subcategories from the analyzed papers by coding each
paper, then organizing codes and continual refinement of
categorization.î It is not clear to the reader what
ìconstant comparison analysisî is and how it is relevant to
this research. They should explicitly motivate the use of
this method.




EXTRA CITATIONS
-	ìEach of these implementations varied greatly in
complexity. For example Markov models could range from
simple first order implementations to complex hidden Markov
modelsî this statement needs citation



\subsection{More extending}
*Extend results interpretation
The results of this paper are informative and as I was
reading them I felt curious to know more. I would have
liked to read more discussion on the trade-offs of the
different algorithmic models in treating emotions (what are
the strengths versus the limitations of different
algorithms). I would also have liked to see some
information about the effect of emotions in HRI with some
results concerning the limitations of the studies and how
we can use these limitations as future research.
Additionally, I would really like to see a critical view of
the authors related to the research they have found. If
there is space in the paper, it would be really good to see
a section o \textbf{Guidelines for research in emotions given the
lessens learners from this paper}



Improve GITHUB



Checkout further:
Paiva, A., Leite, I., Boukricha, H., & Wachsmuth, I.
(2017). Empathy in virtual agents and robots: a survey. ACM
Transactions on Interactive Intelligent Systems (TiiS),
7(3), 1-40.

Leite, I., Martinho, C., & Paiva, A. (2013). Social robots
for long-term interaction: a survey. International Journal
of Social Robotics, 5(2), 291-308.


In Figure 7 it looks like the x axis annotation is shifted
a bit, which makes it very hard to see which label belongs
to which column (I had to count to make sense of the
labels). 





In general, Part C of the discussion was very good and
clear to me, while both part A and B were more difficult to
follow and a bit too brief. Especially since there is some
space left in the end of the paper, I would suggest to add
some more detail to bring the points across more clearly.
For C3, I was wondering if one reason could be that
replication studies are so undervalued in academia in
general. It seems like one cause of action could be to make
replication studies more accepted, which could increase the
number of papers using the same algorithm and / or
methodology with a different robot platform.
In part C, I also think that you can sell the contribution
of this paper better. As I said earlier, I think the
categorization of the papers is very well done and an
excellent step towards developing unified categorization
labels that are adopted in the community. This could
generally help to place ones paper in the related body of
work, but also to make out other relevant publications to
compare ones own approach to



\subsection{Correlations and Contingency Tables}\label{sec:contandlog}
After examining each category individually we created a correlation matrix using the Pearson product-moment correlation coefficients to establish pair-wise correlation (Figure \ref{fig:correlation}). In Figure \ref{fig:correlation} Custom refers to whether the system used a custom model of emotion, while over median refers to using above the median number of emotion categories (such as happy and sad). We found the strongest correlation between input use including emotion stimuli and whether the system was performance or interaction based. We also used contingency tables to compare the system purpose and emotion model (Table \ref{tab:emotiontab} and the purpose with input mapping \ref{tab:inputcat}. These tables show the frequency of custom emotions and each possible mapping in relation to the purpose of emotion in the system. 



\begin{figure}[t]
  \centering
\includegraphics[width=8cm]{images/corr.png}
  \caption{Correlation and Log-Linear Analysis}
  \label{fig:correlation}
\end{figure}



\begin{table}[b]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
            & Custom & Over & Freq \\ \midrule
Performance & Yes    & Yes             & 7    \\
            & Yes    & No              & 45   \\
            & No     & Yes             & 4    \\ \midrule
Interaction & Yes    & Yes             & 36   \\
            & Yes    & No              & 69   \\
            & No     & Yes             & 71   \\ \bottomrule
\end{tabular}
  \caption{Use of Emotional Models by Role of System}
  \label{tab:emotiontab}
\end{table}
